Collaborative Information Dissemination with Graph-based Multi-Agent Reinforcement Learning

Efficient information dissemination is crucial for supporting critical operations across domains like disaster response, autonomous vehicles, and sensor networks. This paper introduces a Multi-Agent Reinforcement Learning (MARL) approach as a significant step forward in achieving more decentralized, efficient, and collaborative information dissemination. We propose a Partially Observable Stochastic Game (POSG) formulation for information dissemination empowering each agent to decide on message forwarding independently, based on the observation of their one-hop neighborhood. This constitutes a significant paradigm shift from heuristics currently employed in real-world broadcast protocols. Our novel approach harnesses Graph Convolutional Reinforcement Learning and Graph Attention Networks (GATs) with dynamic attention to capture essential network features. We propose two approaches, L-DyAN and HL-DyAN, which differ in terms of the information exchanged among agents. Our experimental results show that our trained policies outperform existing methods, including the state-of-the-art heuristic, in terms of network coverage as well as communication overhead on dynamic networks of varying density and behavior.

==> sections/MPR.tex <==
The \gls{olsr}~\cite{rfc3626, rfc7188} protocol is a proactive routing protocol used in \glspl{manet} and, more in general, wireless mesh networks. While being a comprehensive routing protocol implementing different functionalities, \gls{olsr} uses a technique called {\bf \gls{mpr} selection~\cite{994521, adjih:inria-00471715}} to optimize information dissemination throughout a broadcast network. 
The process starts with a bootstrap phase in which the nodes exchange their identity and that of their one-hope neighbors via two rounds of HELLO messages.  MPR selection then uses a third round of HELLO messages, where every node incorporates the identifiers of a specific subset of its neighbors known as the \gls{mpr} set. This set comprises of only those neighbors that are chosen to forward the packages sent by the node.
The \gls{mpr} selection algorithm ensures that every node has a minimal set of \gls{mpr} nodes that cover all its two-hop neighbors using a heuristic  based on the graph-theoretic notion of dominating set (see Section \ref{})to minimize the number of transmissions needed to spread information. 
In its default implementation~\cite{rfc3626}, each node selects neighbors with the largest number of two-hop neighbors in common with it. 
The complete \gls{mpr} selection algorithm used by \gls{olsr} is shown in Algorithm~\ref{alg:mpr-selection} in Section \ref{sec:mpr-pseudo} of the Supplementary Materials. 


requires all nodes to send multiple rounds of HELLO messages. A first round allows nodes to mutually detect one-hop neighbors and a second round enables the 
exchange their respective current neighborhood information. 
During the third round of exchanging HELLO messages, every node incorporates the identifiers of a specific subset of its neighbors known as the \gls{mpr} set. This set comprises of only those neighbors that are chosen to forward the packages sent by the node.
The \gls{mpr} selection algorithm ensures that every node has a minimal set of \gls{mpr} nodes that cover all its two-hop neighbors using a heuristic  to minimize the number of transmissions needed to spread information. 
The selection heuristic is based on the concept of dominating set (Definition 1) and, in its default implementation~\cite{rfc3626}, each node selects neighbors with the largest number of two-hop neighbors in common with it.
The complete \gls{mpr} selection algorithm used by \gls{olsr} is shown in Algorithm~\ref{alg:mpr-selection} in Section \ref{sec:mpr-pseudo} of the Supplementary Materials. 
It is worth mentioning that mechanisms of forwarding \enquote{willingness} can also be enabled in the protocol, but such an option does not fall in the scope of this work. 



==> sections/policy_parameterization.tex <==
In our proposed architecture, the local observation $\mathcal{O}_i(t)$ for each active agent $i \in \mathcal{[I]}_a$ is fed into an encoder consisting of a multi-headed \gls{gat}~\cite{veličković2018graph} with dynamic attention~\cite{brody2022how}. The intuition behind choosing a \gls{gat} architecture is that every neighbor in some agent's $i$ neighborhood $\mathcal{N}_i$ will have a different attention score. 

Given the local observation of some agent $i$ the output for each attention head $m \in M$ will be:

\[
\mathbf{x}^{m}_i = \alpha^m_{i,i}\mathbf{W}\mathbf{x}_{i} +
\sum_{j \in \mathcal{N}(i)}\alpha^m_{i,j}\mathbf{W}\mathbf{x}_{j}
\forall m \in M\]

We will denote $\mathbf{\hat{X_i}} = \mathbf{x}^0_i||\mathbf{x}^1_i||...||\mathbf{x}^m_i$, where $||$ is the concatenation operator, as the concatenation of every attention output. The dynamic attention $\alpha^m$ for the tuple $(i, j)$ is computed by: 

\[
\alpha^m_{i,j} =
\frac{
\exp\left(\mathbf{a}^{\top}\mathrm{LeakyReLU}\left(\mathbf{W}
[\mathbf{x}_i \, \Vert \, \mathbf{x}_j]
\right)\right)}
{\sum_{k \in \mathcal{N}_i \cup \{ i \}}
\exp\left(\mathbf{a}^{\top}\mathrm{LeakyReLU}\left(\mathbf{W}
[\mathbf{x}_i \, \Vert \, \mathbf{x}_k]
\right)\right)}.
\]

The final latent representation can be expressed as:

\[\mathbf{h_i} = \mathrm{ReLU}(\mathrm{max}_{n \in N_i} \, \mathbf{\hat{X}}_n)\]

Such representation is fed to a decoder which will be responsible to computing the 


    


==> tables/results_steps.tex <==
\small
\begin{tabularx}{\columnwidth}{l|c|c|c|c|c}
\hline
\multicolumn{2}{l|}{Nodes Velocity $\left( \mathrm{units}/\mathrm{step} \right)$}         & 0      & 1      & 6       &10     \\ \hline
\multirow{2}{*}{MPR}               & Messages    &           &           &         &   \\ 
                                   & Coverage   &           &           &          &    \\ \hline
\multirow{2}{*}{DGN}               & Messages   &           &           &          &    \\
                                   & Coverage   &           &           &          &    \\ \hline 
\multirow{2}{*}{L-DyAN}            & Messages   &           &           &          &    \\
                                   & Coverage   &           &           &          &    \\ \hline 
\multirow{2}{*}{HL-DyAN}           & Messages   &           &           &          &    \\ 
                                   & Coverage   &           &           &          &    \\ \hline
\end{tabularx}

